Moving Fast With Broken Data

Machine learning (ML) models in production pipelines are frequently retrained on the latest partitions of large, continually-growing datasets. Due to engineering bugs, partitions in such datasets almost always have some corrupted features; thus, it's critical to detect data issues and block retraining before downstream ML model accuracy decreases. However, it's difficult to identify when a partition is corrupted enough to block retraining. Blocking too often yields stale model snapshots in production; blocking too little yields broken model snapshots in production. In this paper, we present an automatic data validation system for ML pipelines implemented at Meta. We employ what we call a Partition Summarization (PS) approach to data validation: each timestamp-based partition of data is summarized with data quality metrics, and summaries are compared to detect corrupted partitions. We describe how we can adapt PS for several data validation methods and compare their pros and cons. Since none of the methods by themselves met our requirements for high precision and recall in detecting corruptions, we devised GATE, our high-precision and recall data validation method. GATE gave a 2.1x average improvement in precision over the baseline on a case study with Instagram's data. Finally, we discuss lessons learned from implementing data validation for Meta's production ML pipelines.

==> figs/mainresults.tex <==
\begin{table}[h]
\centering
    \begin{subtable}[h]{\linewidth}
    \centering
    % \resizebox{\linewidth}{!}
    {\begin{tabular}{lYY|cc|cc}
\toprule
{} & \multicolumn{2}{Y|}{\textbf{auc}} & \multicolumn{2}{c|}{\textbf{AP}} & \multicolumn{2}{c}{\textbf{precision@0.9}} \\
{} &         $p=1$ &         $p=2$ &             $p=1$ &         $p=2$ &             $p=1$ &         $p=2$ \\
\% history &           &           &               &           &               &           \\
\midrule
0.1 &  0.887218 &  0.932331 &      0.759066 &  0.840136 &      0.538462 &  0.700000 \\
0.2 &  0.924812 &  0.954887 &      0.807236 &  0.897619 &      0.636364 &  0.700000 \\
0.3 &  0.909774 &  0.954887 &      0.780612 &  0.897619 &      0.583333 &  0.700000 \\
0.4 &  0.932331 &  0.939850 &      0.816327 &  0.833333 &      0.700000 &  0.700000 \\
 0.5 &  0.924812 &  0.932331 &      0.816667 &  0.824242 &      0.583333 &  0.636364 \\
 0.6 &  0.947368 &  0.947368 &      0.844444 &  0.844444 &      0.777778 &  0.777778 \\
 \textcolor{red}{0.7} &  \textcolor{red}{0.962406} &   \textcolor{red}{0.962406} &       \textcolor{red}{0.873639} &   \textcolor{red}{0.873639} &       \textcolor{red}{0.875000} &   \textcolor{red}{0.875000} \\
0.8 &  0.954887 &  0.962406 &      0.859751 &  0.873639 &      0.777778 &  0.875000 \\
 0.9 &  0.962406 &  0.962406 &      0.873639 &  0.873639 &      0.875000 &  0.875000 \\
1.0 &  0.962406 &  0.962406 &      0.873639 &  0.873639 &      0.875000 &  0.875000 \\
\bottomrule
\end{tabular}}
\caption{Metrics for $\mathcal{D}_1$}
    \label{tab:ourmethod1}
    \end{subtable} \hfill \begin{subtable}[h]{\linewidth}
    \centering
    % \resizebox{\linewidth}{!}
    {\begin{tabular}{lYY|cc|cc}
\toprule
{} & \multicolumn{2}{Y|}{\textbf{auc}} & \multicolumn{2}{c|}{\textbf{AP}} & \multicolumn{2}{c}{\textbf{precision@0.9}} \\
{} &         $p=1$ &         $p=2$ &             $p=1$ &         $p=2$ &             $p=1$ &         $p=2$ \\
\% history &           &           &               &           &               &           \\
\midrule
0.1 &  0.622807 &  0.750000 &      0.673670 &  0.739080 &      0.678571 &  0.791667 \\
\textcolor{red}{0.2} &  \textcolor{red}{0.640351} &  \textcolor{red}{0.741228} &      \textcolor{red}{0.680040} &  \textcolor{red}{0.730462} &      \textcolor{red}{0.760000} &  \textcolor{red}{0.791667} \\
0.3 &  0.640351 &  0.723684 &      0.673461 &  0.734294 &      0.760000 &  0.791667 \\
0.4 &  0.561404 &  0.622807 &      0.610649 &  0.637687 &      0.730769 &  0.760000 \\
0.5 &  0.561404 &  0.583333 &      0.613855 &  0.620149 &      0.730769 &  0.760000 \\
0.6 &  0.548246 &  0.552632 &      0.627535 &  0.606947 &      0.678571 &  0.730769 \\
0.7 &  0.478070 &  0.504386 &      0.606334 &  0.581326 &      0.612903 &  0.703704 \\
0.8 &  0.385965 &  0.521930 &      0.572164 &  0.589734 &      0.612903 &  0.703704 \\
0.9 &  0.394737 &  0.289474 &      0.574556 &  0.496752 &      0.612903 &  0.612903 \\
1.0 &  0.394737 &  0.289474 &      0.574556 &  0.496752 &      0.612903 &  0.612903 \\
\bottomrule
\end{tabular}}
    \caption{Metrics for $\mathcal{D}_2$}
    \label{tab:ourmethod2}
\end{subtable}
    \caption{Average precision (AP) and precision@0.9 for \gate, based on the fraction of historical statistics vectors used in the nearest neighbors method. We compute distances between statistics vectors using the $\ell_p$ distance measure, for $p=1$ (Manhattan distance) and $p=2$ (Euclidean distance).}
    \label{tab:ourmethod}
\end{table}
